MoViNets: Mobile Video Networks for Efficient Video Recognition

We present Mobile Video Networks (MoViNets), a family of computation and memory efficient video networks that can operate on streaming video for online inference. 3D convolutional neural networks (CNNs) are accurate at video recognition but require large computation and memory budgets and do not support online inference, making them difficult to work on mobile devices. We propose a three-step approach to improve computational efficiency while substantially reducing the peak memory usage of 3D CNNs. First, we design a video network search space and employ neural architecture search to generate efficient and diverse 3D CNN architectures. Second, we introduce the Stream Buffer technique that decouples memory from video clip duration, allowing 3D CNNs to embed arbitrary-length streaming video sequences for both training and inference with a small constant memory footprint. Third, we propose a simple ensembling technique to improve accuracy further without sacrificing efficiency. These three progressive techniques allow MoViNets to achieve state-of-the-art accuracy and efficiency on the Kinetics, Moments in Time, and Charades video action recognition datasets. For instance, MoViNet-A5-Stream achieves the same accuracy as X3D-XL on Kinetics 600 while requiring 80% fewer FLOPs and 65% less memory. Code will be made available at https://github.com/tensorflow/models/tree/master/official/vision.

==> Mobile Video Networks Arxiv/sections/01_intro.tex <==
\begin{figure}[t]
    \begin{center}
    \includegraphics[width=1.0\linewidth]{images/movinet_k600_flops_comparison_v5.pdf}
    \end{center}
        \vspace{-5pt}
        \caption{
            {\bf Accuracy vs. FLOPs and Memory on Kinetics 600}.
            \ournets are more accurate than 2D networks and more efficient than 3D networks.
            Top (log scale): \ournet-A2 achieves {\bf 6\% higher} accuracy than MobileNetV3~\cite{howard2019searching} at the same FLOPs while \ournet-A6 achieves state-of-the-art 83.5\% accuracy being {\bf 5.1x faster} than X3D-XL~\cite{feichtenhofer2020x3d}.
            Bottom: Streaming \ournets require {\bf 10x less memory} at the cost of 1\% accuracy.
            Note that we only train on the ~93\% of Kinetics 600 examples that are available at the time of writing.
            Best viewed in color.
        }
        \vspace{-12pt}
    \label{fig:k600-comparison}
\end{figure}

Efficient video recognition models are opening up new opportunities for mobile camera, IoT, and self-driving applications where efficient and accurate on-device processing is paramount.
Despite recent advances in deep video modeling, it remains difficult to find models that run on mobile devices and achieve high video recognition accuracy.
On the one hand, 3D convolutional neural networks (CNNs)~\cite{tran2018closer, wang2018non, feichtenhofer2019slowfast, feichtenhofer2020x3d, ryoo2019assemblenet} offer state-of-the-art accuracy, but consume copious amounts of memory and computation.
On the other hand, 2D CNNs~\cite{lin2019tsm, zhu2020faster} require far fewer resources suitable for mobile and can run online using frame-by-frame prediction, but fall short in accuracy.

Many operations that make 3D video networks accurate (e.g., temporal convolution, non-local blocks~\cite{wang2018non}, etc.) require all input frames to be processed at once, limiting the opportunity for accurate models to be deployed on mobile devices.
The recently proposed X3D networks~\cite{feichtenhofer2020x3d} provide a significant effort to increase the efficiency of 3D CNNs.
However, they require large memory resources on large temporal windows which incur high costs, or small temporal windows which reduce accuracy.
Other works aim to improve 2D CNNs' accuracy using temporal aggregation~\cite{lin2019tsm, fan2019more, wu2020dynamic, liu2020tam, fan2020rubiksnet}, however their limited inter-frame interactions reduce these models' abilities to adequately model long-range temporal dependencies like 3D CNNs.

This paper introduces {\it three progressive steps} to design efficient video models which we use to produce Mobile Video Networks ({\bf \ournets}), a family of memory and computation efficient 3D CNNs.
%We introduce our methods as follows:

\begin{enumerate}
    \item We first define a {\bf \ournet search space} to allow Neural Architecture Search (NAS) to efficiently trade-off spatiotemporal feature representations.
    \item We then introduce {\bf Stream Buffers} for \ournets, which process videos in small consecutive subclips, requiring constant memory without sacrificing long temporal dependencies, and which enable online inference.
    \item Finally, we create {\bf Temporal Ensembles} of streaming \ournets, regaining the slightly lost accuracy from the stream buffers.
\end{enumerate}

First, we design the \ournet search space to explore how to mix spatial, temporal, and spatiotemporal operations such that NAS can find optimal feature combinations to trade-off efficiency and accuracy.
Figure~\ref{fig:k600-comparison} visualizes the efficiency of the generated \ournets.
\ournet-A0 achieves similar accuracy to MobileNetV3-large+TSM~\cite{howard2019searching, lin2019tsm} on Kinetics 600~\cite{kay2017kinetics} with 75\% fewer FLOPs.
\ournet-A6 achieves state-of-the-art 83.5\% accuracy, 1.6\% higher than X3D-XL~\cite{feichtenhofer2020x3d}, requiring 60\% fewer FLOPs.

Second, we create streaming \ournets by introducing the stream buffer to reduce memory usage from linear to constant in the number of input frames for both training and inference, allowing \ournets to run with substantially fewer memory bottlenecks.
E.g., the stream buffer reduces \ournet-A5's memory usage by 90\%.
In contrast to traditional multi-clip evaluation (test-time data augmentation) approaches~\cite{simonyan2014two, wang2015towards} which also reduce memory, a stream buffer carries over temporal dependencies between consecutive non-overlapping subclips by caching feature maps at subclip boundaries.
The stream buffer allows for a larger class of operations to enhance online temporal modeling than the recently proposed temporal shift~\cite{lin2019tsm}.
We equip the stream buffer with temporally unidirectional causal operations like causal convolution~\cite{oord2016wavenet}, cumulative pooling, and causal squeeze-and-excitation~\cite{hu2018squeeze} with positional encoding to force temporal receptive fields to look only into past frames, enabling \ournets to operate incrementally on streaming video for online inference.
However, the causal operations come at a small cost, reducing accuracy on Kinetics 600 by 1\% on average.

Third, we temporally ensemble \ournets, showing that they are more accurate than single large networks while achieving the same efficiency.
We train two streaming \ournets independently with the same total FLOPs as a single model and average their logits.
This simple technique gains back the loss in accuracy when using stream buffers.

Taken together, these three techniques create \ournets that are high in accuracy, low in memory usage, efficient in computation, and support online inference.
We search for \ournets using the Kinetics 600 dataset~\cite{carreira2018short} and test them extensively on Kinetics 400~\cite{kay2017kinetics}, Kinetics 700~\cite{carreira2019short}, Moments in Time~\cite{monfort2019moments}, Charades~\cite{sigurdsson2016hollywood}, and Something-Something~V2~\cite{goyal2017something}.


==> Mobile Video Networks Arxiv/sections/02_related_work.tex <==
% \vspace{-10pt}
\paragraph{Efficient Video Modeling.}

Deep neural networks have made remarkable progress for video understanding~\cite{ji20123d,simonyan2014two,tran2015learning, wang2016temporal,carreira2017quo, wang2018non,qiu2019learning,feichtenhofer2020x3d,feichtenhofer2019slowfast}.
They extend 2D image models with a temporal dimension, most notably incorporating 3D convolution~\cite{ji20123d,taylor2010convolutional,tran2015learning,xie2017rethinking,hara2018can,qiu2017learning,jiang2019stm,ryoo2019assemblenet}.
% including optical flow as a separate stream to capture motion information~\cite{simonyan2014two,carreira2017quo,feichtenhofer2016convolutional,crasto2019mars,ryoo2019assemblenet}
% Recently, learning with large-scale unlabeled data~\cite{duan2020omni,ghadiyaram2019large,tran2019video} and NAS~\cite{feichtenhofer2020x3d,piergiovanni2020tiny,ryoo2019assemblenet} are used to further improve video understanding.

Improving the efficiency of video models has gained increased attention~\cite{feichtenhofer2019slowfast,tran2019video,feichtenhofer2017spatiotemporal,feichtenhofer2020x3d,lin2019tsm,fan2019more,bhardwaj2019efficient,chen2018big,li2020smallbignet,piergiovanni2020tiny}.
% Several works made progress on producing video models suitable for mobile applications.
Some works explore the use of 2D networks for video recognition by processing videos in smaller segments followed by late fusion~\cite{karpathy2014large,donahue2015long,yue2015beyond,wang2016temporal,feichtenhofer2017spatiotemporal,sun2017lattice,li2018recurrent,li2018videolstm,wang2018non,zhou2018temporal,zhu2020faster}. 
% Temporal Relation Networks (TRN)~\cite{zhou2018temporal} by applying relational networks to model the temporal relations.
% Other works use early fusion to aggregate intermediate feature representations~\cite{zolfaghari2018eco, fan2019more, fan2020rubiksnet, wu2020dynamic}.
The Temporal Shift Module~\cite{lin2019tsm} uses early fusion to shift a portion of channels along the temporal axis, boosting accuracy while supporting online inference.
% Our stream buffer approach is a generalization of TSM, allowing more types of operations across more frames (e.g., CausalConv) to enhance temporal modeling.

% Another line of work considers separate convolutions to reduce intensive computation in 3D convolution~\cite{fan2019more,chen2018big,li2020smallbignet,feichtenhofer2019slowfast,xie2018rethinking,tran2018closer,qiu2017learning,tran2019video}. 
% Some of them interleave the video frames by a heavy network to capture spatial semantics and a lightweight network to capture temporal motion~\cite{fan2019more,chen2018big,li2020smallbignet,feichtenhofer2019slowfast}. Others decompose the 3D convolution into the combination of 2D spatial and 1D temporal convolution~\cite{qiu2017learning,tran2018closer,xie2018rethinking}. 
% Alternatively, they bring techniques (e.g., depthwise convolution) from mobile image models to video models~\cite{tran2019video,feichtenhofer2020x3d,piergiovanni2020tiny,zolfaghari2018eco, fan2019more, zhu2020faster, fan2020rubiksnet, wu2020dynamic}.

\vspace{-12pt}
\paragraph{Causal Modeling.}
WaveNet~\cite{oord2016wavenet} introduces causal convolution, where the receptive field of a stack of 1D convolutions only extends to features up to the current time step.
We take inspiration from other works using causal convolutions~\cite{carreira2018massively,chang2018temporal,dai2019transformer,cheng2019sparse,daiya2020stock} to design stream buffers for online video model inference, allowing frame-by-frame predictions with 3D kernels.
% Similarly, Transformer-XL~\cite{dai2019transformer} caches activations for improved accuracy in long-range sequence modeling.

\vspace{-12pt}
\paragraph{Multi-Objective NAS.}
The use of NAS~\cite{zoph2016neural,liu2018progressive,pham2018efficient,tan2019mnasnet,cai2018proxylessnas,kandasamy2018neural} with multi-objective architecture search has also grown in interest, producing more efficient models in the process for image recognition~\cite{tan2019mnasnet, cai2018proxylessnas, bender2020can} and video recognition~\cite{piergiovanni2020tiny, ryoo2019assemblenet}.
We make use of TuNAS~\cite{bender2020can}, a one-shot NAS framework which uses aggressive weight sharing that is well-suited for computation intensive video models.

\vspace{-12pt}
\paragraph{Efficient Ensembles.}
Deep ensembles are widely used in classification challenges to boost the performance of CNNs~\cite{bian2017revisiting,simonyan2014very,Szegedy_2015_CVPR,he2016deep}.
% and it is also introduced for uncertainty estimation~\cite{lakshminarayanan2017simple,he2020bayesian}.
More recent results indicate that deep ensembles of small models can be more efficient than single large models on image classification~\cite{kondratyuk2020ensembling,lobacheva2020power,NIPS2016_c51ce410, NIPS2016_20d135f0,furlanello2018born}, and we extend these findings to video classification.


==> Mobile Video Networks Arxiv/sections/03_approach.tex <==
This section describes our progressive three-step approach to \ournets.
We first detail the design space to search for \ournets.
Then we define the stream buffer and explain how it reduces the networks' memory footprints, followed by the temporal ensembling to improve accuracy.

%------------------------------------------------------------------------
\subsection{Searching for \ournet} \label{sec:nas}
Following the practice of 2D mobile network search~\cite{tan2019mnasnet, tan2019efficientnet}, we start with the TuNAS framework~\cite{bender2020can}, which is a scalable implementation of one-shot NAS with weight sharing on a supernetwork of candidate models, and repurpose it for 3D CNNs for video recognition.
We use Kinetics 600~\cite{kay2017kinetics} as the video dataset to search over for all of our models, consisting of 10-second video sequences each at 25fps for a total of 250 frames.

\begin{table}[t]
    \footnotesize
    % Architecture diagram commands
    \newcommand{\blocks}[3]{
        \multirow{3}{*}{
            \(\left[
            \begin{array}{c}
                \text{1$\times$1$^\text{2}$, #2}\\[-.1em] 
                \text{1$\times$3$^\text{2}$, #2}\\[-.1em] 
                \text{1$\times$1$^\text{2}$, #1}
            \end{array}
            \right]\)$\times$#3
        }
    }
    \newcommand{\blocket}[4]{\multirow{3}{*}{\(\left[\begin{array}{c}\text{1$\times$1$^\text{2}$, #1}\\[-.1em] \text{$3$$\times$3$^\text{2}$, #2}\\[-.1em] \text{1$\times$1$^\text{2}$, #3}\end{array}\right]\)$\times$#4}
    }
    \newcommand{\blockt}[3]{\multirow{3}{*}{\(\left[\begin{array}{c}\text{\underline{3$\times$1$^\text{2}$}, #2}\\[-.1em] \text{1$\times$3$^\text{2}$, #2}\\[-.1em] \text{1$\times$1$^\text{2}$, #1}\end{array}\right]\)$\times$#3}
    }
    \newcommand{\blockseq}[3]{\text{#1$\times$#2$^\text{2}$, #3}\\[-.1em]}

    \begin{center}
 
    \begin{tabularx}{\columnwidth}{@{}Xcc@{}}
            \toprule
            \sc Stage & \sc Network Operations & \sc Output size \\
            \midrule
            data & stride $\tau$, RGB & $T\times S^\text{2}$ \\
            conv$_1$ & \multicolumn{1}{c}{$1\times k_1^\text{2}$, $c_1$}
            & $T\times \frac{S^\text{2}}{2}$ \\
            \midrule
            \multirow{2}{*}{block$_2$} & \multirow{2}{*}{
                \(\left[
                \begin{array}{c}
                    \blockseq{{$k_{2}^{\text{time}}$}}{{$(k_{2}^{\text{space}})$}}{{$c_2^\text{base}$, $c_2^\text{expand}$}}
                \end{array}
                \right]\)$\times L_2$} & 
                \multirow{2}{*}{$T\times \frac{S^\text{2}}{4}$}  \\
            & & \\
            & $\cdots$ & \\
            \multirow{2}{*}{block$_n$} & \multirow{2}{*}{
                \(\left[
                \begin{array}{c}
                    \blockseq{{$k_{n}^{\text{time}}$}}{{$(k_{n}^{\text{space}})$}}{{$c_n^\text{base}$, $c_n^\text{expand}$}}
                \end{array}
                \right]\)$\times L_n$} &
                \multirow{2}{*}{$T\times \frac{S^\text{2}}{2^n}$}  \\
            & & \\
            \midrule
            conv$_{n+1}$ & \multicolumn{1}{c}{$1\times1^\text{2}$, {$c_{n+1}^\text{base}$}}
            & $T\times \frac{S^\text{2}}{2^n}$ \\
            pool$_{n+2}$ & \multicolumn{1}{c}{$T\times \frac{S^\text{2}}{2^n}$}
            & $1\times1^\text{2}$ \\
            dense$_{n+3}$ & \multicolumn{1}{c}{$1\times1^\text{2}$, {$c_{n+3}^\text{base}$}}
            & $1\times1^\text{2}$ \\
            dense$_{n+4}$ & \multicolumn{1}{c}{$1\times1^\text{2}$, {\# classes}}
            & $1\times1^\text{2}$ \\
            \bottomrule
    \end{tabularx}

    \end{center}
    \vspace{-2pt}
    \caption{
        {\bf \ournet Search Space}. 
        Given an input video with $T$ frames and resolution $S^\text{2}$, at stage $i$ we search over base widths $c_i^{\text{base}}$ and the number of layers $L_i$ in the block.
        Within each layer we search for expansion widths $c_i^{\text{expand}}$, along with 3D convolutional kernel sizes $k_{i}^{\text{time}}\times(k_{i}^{\text{space}})^2 \in \{1, 3, 5, 7\} \times \{1, 3, 5, 7\}^2$.
    }
    \label{table:nas-ssd}
    \vspace{-5pt}
\end{table}


\vspace{-10pt}
\paragraph{\ournet Search Space.}
We build our base search space on MobileNetV3~\cite{howard2019searching}, which provides a strong baseline for mobile CPUs.
It consists of several blocks of inverted bottleneck layers with varying filter widths, bottleneck widths, block depths, and kernel sizes per layer. 
Similar to X3D~\cite{feichtenhofer2020x3d}, we expand the 2D blocks in MobileNetV3 to deal with 3D video input.
Table~\ref{table:nas-ssd} provides a basic overview of the search space, detailed as follows.

We denote by $T \times S^2 = 50 \times 224^2$ and $\tau = 5$ (5fps) the dimensions and frame stride, respectively, of the input to the target \ournets.
For each block in the network, we search over the base filter width $c^{\text{base}}$ and the number of layers $L \leq 10$ to repeat within the block. We apply multipliers $\{0.75, 1, 1.25\}$ over the feature map channels within every block, rounded to a multiple of 8. 
We set $n = 5$ blocks, with strided spatial downsampling for the first layer in each block except the 4th block (to ensure the last block has spatial resolution $7^2$).
The blocks progressively increase their feature map channels: $\{16, 24, 48, 96, 96, 192\}$.
The final convolution layer's base filter width is $512$, followed by a $2048$D dense layer before the classification layer.

With the new time dimension, we define the 3D kernel size within each layer, $k^{\text{time}}\times(k^{\text{space}})^2$, to be chosen as one of the following: \{1x3x3, 1x5x5, 1x7x7, 5x1x1, 7x1x1, 3x3x3, 5x3x3\} (we remove larger kernels from consideration).
These choices enable a layer to focus on and aggregate different dimensional representations, expanding the network's receptive field in the most pertinent directions while reducing FLOPs along other dimensions.
Some kernel sizes may benefit from having different numbers of input filters, so we search over a range of bottleneck widths $c^{\text{expand}}$ defined as multipliers in $\{1.5, 2.0, 2.5, 3.0, 3.5, 4.0\}$ relative to $c^{\text{base}}$.
Each layer surrounds the 3D convolution with two 1x1x1 convolutions to expand and project between $c^{\text{base}}$ and $c^{\text{expand}}$.
We do not apply any temporal downsampling to enable frame-wise prediction.

Instead of applying spatial squeeze-and-excitation (SE)~\cite{hu2018squeeze}, we use SE blocks to aggregate spatiotemporal features via 3D average pooling, applying it to every bottleneck block as in \cite{howard2019searching, tan2019efficientnet}.
We allow SE to be searchable, optionally disabling it to conserve FLOPs.

\vspace{-10pt}
\paragraph{Scaling the Search Space.}
Our base search space forms the basis for \ournet-A2.
For the other \ournets, we apply a compound scaling heuristic similar to the one used in EfficientNet~\cite{tan2019efficientnet}.
The major difference in our approach is that we scale the {\it search space} itself rather than a single model (i.e., search spaces for models A0-A5).
Instead of finding a good architecture and then scaling it, we search over all scalings of all architectures, broadening the range of possible models.

We use a small random search to find the scaling coefficients (with an initial target of 300 MFLOPs per frame), which roughly double or halve the expected size of a sampled model in the search space.
For the choice of coefficients, we resize the base resolution $S^2$, frame stride $\tau$, block filter width $c^{\text{base}}$, and block depths $L$.
We perform the search on different FLOPs targets to produce a family of models ranging from MobileNetV3-like sizes up to the sizes of ResNet3D-152~\cite{he2016deep, hara2018can}.
Appendix~\appendixsearchspace provides more details of the search space, the scaling technique, and a description of the search algorithm. 

The \ournet search space gives rise to a family of versatile networks, which outperform state-of-the-art efficient video recognition CNNs on popular benchmark datasets.
However, their memory footprints grow proportionally to the number of input frames, making them difficult to handle long videos on mobile devices.
The next subsection introduces a stream buffer to reduce the networks' memory consumption from linear to constant in video length.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/streaming_eval_horizon.pdf}
    \caption{
        {\bf Streaming Evaluation vs. Multi-Clip Evaluation}.
        In multi-clip evaluation (a type of test-time data augmentation), we embed overlapping subclips of an input video with 3D convolutions and average the logits.
        In streaming evaluation, we use the stream buffer to carry forward input features between non-overlapping subclips and apply causal operations, thereby allowing the temporal receptive field to cover the whole video.
        This stream buffer increases accuracy while retaining the benefits of reduced memory from multi-clip evaluation.
        % In this example, we use a temporal kernel size of 3, resulting in padding and buffer sizes of 2.
    }
    \label{fig:multi-clip-vs-stream-buffer}
    \vspace{-10pt}
\end{figure*}

%------------------------------------------------------------------------
\subsection{The Stream Buffer with Causal Operations} \label{sec:stream-buffer}
Suppose we have an input video $\vec{x}$ with $T$ frames that may cause a model to exceed a set memory budget.
A common solution to reduce memory is  multi-clip evaluation~\cite{simonyan2014two, wang2015towards}, where the model averages predictions across $n$ overlapping subclips with $T^{\text{clip}} < T$ frames each, as seen in Figure~\ref{fig:multi-clip-vs-stream-buffer} (left).
It reduces memory consumption to $O(T^{\text{clip}})$.
However, it poses two major disadvantages: 
1) It limits the temporal receptive fields to each subclip and ignores long-range dependencies, potentially harming accuracy.
2) It recomputes frame activations which overlap, reducing efficiency.

\vspace{-10pt}
\paragraph{Stream Buffer.}
To overcome the above mentioned limitations, we propose stream buffer as a mechanism to cache feature activations on the boundaries of subclips, allowing us to expand the temporal receptive field across subclips and requiring no recomputation, as shown in Figure~\ref{fig:multi-clip-vs-stream-buffer} (right).

Formally, let $\vec{x}_{i}^{\text{clip}}$ be the current subclip (raw input or activation) at step $i < n$, where we split the video into $n$ adjacent \emph{non-overlapping} subclips  of length $T^\text{clip}$ each.
We start with a zero-initialized tensor representing our buffer $B$ with length $b$ along the time dimension and whose other dimensions match $\vec{x}_{i}^{\text{clip}}$. We compute the feature map $F_{i}$ of the buffer concatenated~($\oplus$) with the subclip along the time dimension as:
\begin{align}
    F_{i} = f(B_{i} \oplus \vec{x}_{i}^{\text{clip}})
\end{align}
where $f$ represents a spatiotemporal operation (e.g., 3D convolution).
When processing the next clip, we update the contents of the buffer to: 
\begin{align}
    B_{i+1} = (B_{i} \oplus \vec{x}_{i}^{\text{clip}})_{[-b:]}
\end{align}
where we denote $[-b:]$ as a selection of the last $b$ frames of the concatenated input.
As a result, our memory consumption is dependent on $O(b + T^{\text{clip}})$, which is constant as the total video frames $T$ or number of subclips $n$ increase.

\vspace{-10pt}
\paragraph{Relationship to TSM.}
The Temporal Shift Module (TSM)~\cite{lin2019tsm} can be seen as a special case of the stream buffer, where $b = 1$ and $f$ is an operation that shifts a proportion of channels in the buffer $B_t = \vec{x}_{t-1}$ to the input $\vec{x}_{t}$ before computing a spatial convolution at frame $t$.

\vspace{-2pt}
\subsubsection{Causal Operations}
A reasonable approach to fitting 3D CNNs' operations to the stream buffer is to enforce \emph{causality}, i.e., any features must not be computed  from future frames.
This has a number of advantages, including the ability to reduce a subclip $\vec{x}_i^{\text{clip}}$ down to a single frame without affecting activations or predictions, and enables 3D CNNs to work on streaming video for online inference.
While it is possible to use non-causal operations, e.g., buffering in both temporal directions, we would lose online modeling capabilities which is a desirable property for mobile.

\vspace{-10pt}
\paragraph{Causal Convolution (CausalConv).}
By leveraging the translation equivariant property of convolution, we replace all temporal convolutions with CausalConvs~\cite{oord2016wavenet}, effectively making them unidirectional along the temporal dimension.
Concretely, we first compute padding to balance the convolution across all axes and then move any padding after the final frame and merge it with any padding before the first frame.
% Figure~\ref{fig:causal-conv} illustrates the effect of padding on CausalConv.
See Appendix~\appendixmoreresults for an illustration of how the receptive field differs from standard convolution, as well as a description of the causal padding algorithm.

When using a stream buffer with CausalConv, we can replace causal padding with the buffer itself, carrying forward the last few frames from a previous subclip and copying them into the padding of the next subclip.
If we have a temporal kernel size of $k$ (and we do not use any strided sampling), then our padding and therefore buffer width becomes $b = k - 1$. 
Usually, $k = 3$ which implies $b = 2$, resulting in a small memory footprint.
Stream buffers are only required before layers that aggregate features across multiple frames, so spatial and pointwise convolutions (e.g., 1x3x3, 1x1x1) can be left as-is, further saving memory.

\vspace{-10pt}
\paragraph{Cumulative Global Average Pooling (CGAP).}
We use CGAP to approximate any global average pooling involving the temporal dimension.
For any activations up to frame $T'$, we can compute this as a cumulative sum:
\begin{align}
    \operatorname{CGAP}(\vec{x}, T') = \frac{1}{T'} \sum_{t=1}^{T'} \vec{x}_t,
\end{align}
where $\vec{x}$ represents a tensor of activations. 
To compute CGAP causally, we keep a single-frame stream buffer storing the cumulative sum up to $T'$.
% Our streaming models use CGAP for SE and for the final pooling layer.

\vspace{-10pt}
\paragraph{CausalSE with Positional Encoding.}
We denote CausalSE as the application of CGAP to SE, where we multiply the spatial feature map at frame $t$ with the SE computed from $\operatorname{CGAP}(\vec{x}, t)$.
From our empirical results, CausalSE is prone to instability likely due to the SE projection layers have a difficult time determining the quality of the CGAP estimate, which has high variance early in the video.
To combat this problem, we apply a sine-based fixed positional encoding (\textsc{PosEnc}) scheme inspired by Transformers~\cite{vaswani2017attention, liu2018intriguing}.
We directly use frame index as the position and sum the vector with CGAP output before applying the SE projection.
% $\operatorname{CausalSE}(\vec{x}, t) = \operatorname{SE}(\operatorname{CGAP}(\vec{x}, t) + \operatorname{PosEnc}(t))$.
% \begin{align}
%     PE_{\omega}(pos) = \sin(pos / \omega)
% \end{align}

\vspace{-2pt}
\subsubsection{Training and Inference with Stream Buffers}

\vspace{-2pt}
\paragraph{Training.}
To reduce the memory requirements during training, we use a recurrent training strategy where we split a given batch of examples into $n$ subclips, applying a forward pass that outputs a prediction for each subclip, using stream buffers to cache activations.
However, we do not backpropagate gradients past the buffer so that the memory of previous subclips can be deallocated.
Instead, we compute losses and accumulate computed gradients between subclips, similar to batch gradient accumulation.
This allows the network to account for all $T = nT^{\text{clip}}$ frames, performing $n$ forward passes before applying the gradients.
This training strategy allows the network to learn longer term dependencies thus results in better accuracy than a model trained with shorter video length (see Appendix~\appendixmoreresults).

We can set $T^{\text{clip}}$ to any value without affecting accuracy.
However, ML accelerators (e.g., GPUs) benefit from multiplying large tensors, so for training we typically set a value of $T^{\text{clip}} \in \{8, 16, 32\}$.
This accelerates training while allowing careful control of memory cost.

\vspace{-10pt}
\paragraph{Online Inference.}
One major benefit of using causal operations like CausalConv and CausalSE is to allow a 3D video CNN to work online.
Similar to training, we use the stream buffer to cache activations between subclips.
However, we can set the subclip length to a single frame ($T^{\text{clip}} = 1$) for maximum memory savings.
This also reduces the latency between frames, enabling the model to output predictions frame-by-frame on a streaming video, accumulating new information incrementally like a recurrent network (RNN)~\cite{hochreiter1997long}.
But unlike traditional convolutional RNNs, we can input a variable number of frames per step to produce the same output.
For streaming architectures with CausalConv, we predict a video's label by pooling the frame-by-frame output features using CGAP.

\subsection{Temporal Ensembles}
The stream buffers can reduce \ournets' memory footprints up to an order of magnitude in the cost of about 1\% accuracy drop on Kinetics 600. 
We can restore this accuracy using a simple ensembling strategy.
We train two \ournets independently with the same architecture, but halve the frame-rate, keeping the temporal duration the same (resulting in half the input frames).
We input a video into both networks, with one network having frames offset by one frame and apply an arithmetic mean on the unweighted logits before applying softmax.
This method results in a two-model ensemble with the same FLOPs as a single model before halving the frame-rate, providing prediction with enriched representations.
In our observations, despite the fact that both models in the ensemble may have lower accuracy than the single model individually, together when ensembled they can have higher accuracy than the single model.


==> Mobile Video Networks Arxiv/sections/04_experiments.tex <==
In this section, we evaluate \ournets' accuracy, efficiency, and memory consumption during inference on five representative action recognition datasets.

\vspace{-10pt}
\paragraph{Datasets.}
We report results on all Kinetics datasets, including Kinetics 400~\cite{carreira2017quo, kay2017kinetics}, Kinetics 600~\cite{carreira2018short}, and Kinetics 700~\cite{carreira2019short}, which contain 10-second, 250-frame video sequences at 25 fps labeled with 400, 600, and 700 action classes, respectively.
We use examples that are available \emph{at the time of writing}, which is 87.5\%, 92.8\%, and 96.2\% of the training examples respectively (see Appendix~\appendixmoreresults).
Additionally, we experiment with Moments in Time~\cite{monfort2019moments}, containing 3-second, 75-frame sequences at 25fps in 339 action classes, and Charades~\cite{sigurdsson2016hollywood}, which has variable-length videos with 157 action classes where a video can contain multiple class annotations.
We include Something-Something V2~\cite{goyal2017something} and Epic Kitchens 100~\cite{damen2020rescaling} results in Appendix~\appendixmoreresults.

\vspace{-10pt}
\paragraph{Implementation Details.} 
For each dataset, all models are trained with RGB frames from scratch, i.e., we do not apply any pretraining.
For all datasets, we train with 64 frames (except when the inference frames are fewer) at various frame-rates, and run inference with the same frame-rate.

We run TuNAS using Kinetics 600 and keep 7 \ournets each having a FLOPs target used in~\cite{feichtenhofer2020x3d}.
As our models get larger, our scaling coefficients increase the input resolution, number of frames, depth, and feature width of the networks.
We also experiment with AutoAugment~\cite{cubuk2018autoaugment} augmentation used in image classification, i.e., we sample a random image augmentation for each video and apply the same augmentation for each frame.
For the architectures of the 7 models as well as training hyperparameters, see Appendix~\appendixarchitectures.

\vspace{-10pt}
\paragraph{Single-Clip vs. Multi-Clip Evaluation.}
We evaluate all our models with a single clip sampled from input video with a fixed temporal stride, covering the entire video duration.
When the single-clip and multi-clip evaluations use the same number of frames in total so that FLOPs are equivalent, we find that single-clip evaluation yields higher accuracy (see Appendix~\appendixmoreresults).
This can be due in part to 3D CNNs being able to model longer-range dependencies, even when evaluating on many more frames than it was trained on.
Since existing models commonly use multi-clip evaluation, we report the total FLOPs per video, not per clip, for a fair comparison.

However, single-clip evaluation can greatly inflate a network's peak memory usage (as seen in Figure~\ref{fig:k600-comparison}), which is likely why multi-clip evaluation is commonly used in previous work.
The stream buffer eliminates this problem, allowing \ournets to predict like they are embedding the full video, and incurs less peak memory than multi-clip evaluation.

We also reproduce X3D~\cite{feichtenhofer2020x3d}, arguably the most related work to ours, to test its performance under single-clip and 10-clip evaluation to provide more insights.
We denote 30-clip to be the evaluation strategy with 10 clips times three spatial crops for each video, while 10-clip just uses one spatial crop.
We avoid any spatial augmentation or temporal sampling in \ournets during inference to improve efficiency.

\vspace{-3pt}
\subsection{Comparison Results on Kinetics 600}
\vspace{-3pt}
\paragraph{\ournets without Stream Buffers.} 
Table~\ref{table:k600-comparison} presents the main results of seven \ournets on Kinetics 600 \emph{before applying the stream buffer}, mainly compared with various X3D models~\cite{feichtenhofer2020x3d}, which are recently developed for efficient video recognition. The columns of the table correspond to the Top-1 classification accuracy; GFLOPs per video a model incurs; resolution of the input video frame (where we shorten $224^2$ to 224); input frames per video, where $30\times4$ means the 30-clip evaluation with 4 frames as input in each run; frames per second (FPS), determined by the temporal stride $\tau$ in the search space for \ournets; and a network's number of parameters.


\begin{table}[tbp]
    \newcommand{\frameinput}[2]{#1$\times$#2$^2$}
    \begin{center}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}lrrrrrr@{}}
    \toprule
        \sc Model & \sc Top-1 & \sc gflops & \sc Res & \sc Frames & \sc FPS & \sc Param \\
    \midrule
        \bf \ournet-A0 & \bf 71.5 & \bf 2.71 & 172 & 1$\times$50 & 5 & 3.1M \\
        MobileNetV3-S* \cite{howard2019searching} & 61.3 & 2.80 & 224 & 1$\times$50 & 5 & 2.5M \\
        MobileNetV3-S+TSM* \cite{lin2019tsm} & 65.5 & 2.80 & 224 & 1$\times$50 & 5 & 2.5M \\
        %X3D-XS \cite{feichtenhofer2020x3d} & 71.4 & 6.03 & \frameinput{4}{182} & 10 & 2 & 3.8M \\
        X3D-XS* \cite{feichtenhofer2020x3d} & 70.2 & 3.88 & 182 & 1$\times$20 & 2 & 3.8M \\
    \midrule
        \bf \ournet-A1 & \bf 76.0 & \bf 6.02 & 172 & 1$\times$50 & 5 & 4.6M \\
        X3D-S* \cite{feichtenhofer2020x3d} & 73.4 & 7.80 & 182 & 1$\times$40 & 4 & 3.8M \\
        X3D-S* \cite{feichtenhofer2020x3d} & 74.3 & 9.75 & 182 & 1$\times$50 & 5 & 3.8M \\
    \midrule
        \bf \ournet-A2 & \bf 77.5 & \bf 10.3 & 224 & 1$\times$50 & 5 & 4.8M \\
        MobileNetV3-L* \cite{howard2019searching} & 68.1 & 11.0 & 224 & 1$\times$50 & 5 & 5.4M \\
        MobileNetV3-L+TSM*~\cite{lin2019tsm} & 71.4 & 11.0 & 224 & 1$\times$50 & 5 & 5.4M  \\
        X3D-XS \cite{feichtenhofer2020x3d} & 72.3 & 23.3 & 182 & 30$\times$4 & 2 & 3.8M \\
        % X3D-S \cite{feichtenhofer2020x3d} & 75.9 & 19.6 & \frameinput{13}{182} & 10 & 4 & \bf 3.8M \\
        X3D-M* \cite{feichtenhofer2020x3d} & 76.9 & 19.4 & 256 & 1$\times$50 & 5 & 3.8M \\
    \midrule
        \bf \ournet-A3 & 80.8 & \bf 56.9 & 256 & 1$\times$120 & 12 & 5.3M \\
        \bf \ournet-A3 + AutoAugment & \bf 81.3 & \bf 56.9 & 256 & 1$\times$120 & 12 & 5.3M \\
        X3D-S \cite{feichtenhofer2020x3d} & 76.4 & 76.1 & 182 & 30$\times$13 & 4 & 3.8M \\
        % X3D-M \cite{feichtenhofer2020x3d} & 77.7 & 62.0 & \frameinput{16}{256} & 10 & 5 & \bf 3.8M \\
        X3D-L* \cite{feichtenhofer2020x3d} & 79.1 & 77.5 & 356 & 1$\times$50 & 5 & 6.1M \\
    \midrule
        \bf \ournet-A4 & 81.2 & \bf 105 & 290 & 1$\times$80 & 8 & 4.9M \\
        \bf \ournet-A4 + AutoAugment & \bf 83.0 & \bf 105 & 290 & 1$\times$80 & 8 & 4.9M \\
        X3D-M \cite{feichtenhofer2020x3d} & 78.8 & 186 & 256 & 30$\times$16 & 5 & 3.8M \\
        % X3D-L \cite{feichtenhofer2020x3d} & 79.4 & 248 & \frameinput{16}{356} & 10 & 5 & 6.1M \\
        X3D-L* \cite{feichtenhofer2020x3d} & 80.7 & 187 & 356 & 1$\times$120 & 2 & 6.1M \\
        X3D-XL* \cite{feichtenhofer2020x3d} & 80.3 & 151 & 356 & 1$\times$50 & 5 & 11.0M \\
        I3D \cite{carreira2018short} & 71.6 & 216 & 224 & 1$\times$250 & 25 & 12M \\
        ResNet3D-50* & 78.7 & 390 & 224 & 1$\times$250 & 25 & 34.0M \\
    \midrule
        \bf \ournet-A5 & 82.7 & \bf 281 & 320 & 1$\times$120 & 12 & 15.7M \\
        \bf \ournet-A5 + AutoAugment & \bf 84.3 & \bf 281 & 320 & 1$\times$120 & 12 & 15.7M \\
        X3D-L \cite{feichtenhofer2020x3d} & 80.5 & 744 & 356 & 30$\times$16 & 5 & 6.1M \\
        % X3D-XL \cite{feichtenhofer2020x3d} & 81.1 & 484 & \frameinput{16}{356} & 10 & 5 & 11.0M \\
    \midrule
        \bf \ournet-A6 & 83.5 & \bf 386 & 320 & 1$\times$120 & 12 & 31.4M \\
        \bf \ournet-A6 + AutoAugment & \bf 84.8 & \bf 386 & 320 & 1$\times$120 & 12 & 31.4M \\
        ViViT-L/16x2~\cite{arnab2021vivit} & 83.0 & 3990 & 320 & 12$\times$32 & 12 & 88.9M \\
        TimeSformer-HR \cite{bertasius2021space} & 82.4  & 5110 & 224 & 3$\times$8 & 1.5 & 120M \\
        X3D-XL \cite{feichtenhofer2020x3d} & 81.9 & 1452 & 356 & 10$\times$16 & 5 & 11.0M \\
        ResNet3D-152* & 81.1 & 1400 & 224 & 1$\times$250 & 25 & 80.1M \\
        ResNet3D-50-G~\cite{li2020perf} & 82.0 & 3666 & 224 & 1$\times$250 & 25 & - \\
        SlowFast-R50 \cite{feichtenhofer2019slowfast} & 78.8 & 1080 & 256 & 30$\times$16 & 5 & 34.4M \\
        SlowFast-R101 \cite{feichtenhofer2019slowfast} & 81.8 & 7020 & 256 & 30$\times$16 & 5 & 59.9M \\
        LGD-R101 \cite{qiu2019learning} & 81.5 & - & 224 & 15$\times$16 & 25 & - \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{
        {\bf Accuracy of \ournet on Kinetics 600}.
        We measure total GFLOPs per video across all frames, and report the inference resolution (res),  number of clips $\times$ frames per clip (frames), and frame rate (fps) of each video clip.
        * denotes our reproduced models.
        For X3D, we report \emph{inference} resolution, which differs from training.
        We report all datapoints to the best knowledge available.
    }
    \label{table:k600-comparison}
    \vspace{-5pt}
\end{table}

% \vspace{-10pt}

%Results demonstrate that our models are not only more efficient than X3D per video, but also more efficient per frame as well (despite the disadvantage of embedding fewer frames).

%A more detailed look on Kinetics 600 can be seen in Table~\ref{table:k600-comparison}.
% We compare all models with G
%To compare with frame-based 2D models, we train MobileNetV3~\cite{howard2019searching} using our training setup, averaging logits across frames.
%Our smallest \ournet-A0 is the same size as MobileNetV3-small while being 10\% more accurate, and similarly for \ournet-A2 and MobileNetV3-large.


\ournet-A0 has fewer GFLOPs and is 10\% more accurate than the frame-based MobileNetV3-S~\cite{howard2019searching} (where we train MobileNetV3 using our training setup, averaging logits across frames). 
\ournet-A0 also outperforms X3D-S in terms of both accuracy and GFLOPs. 
\ournet-A1 matches the GFLOPs of X3D-S, but its accuracy is 2\% higher than X3D-S.

%We also evaluate MobileNetV3-large with TSM~\cite{lin2019tsm} to show that \ournet-A2 still has a distinct advantage in efficiency due to temporal convolutions and searched architecture on video.

Growing the target GFLOPs to the range between X3D-S and 30-clip X3D-XS, we arrive at \ournet-A2. We can achieve a little higher accuracy than 30-clip X3D-XS or X3D-M by using almost half of their GFLOPs.
Additionally, we include the frame-by-frame MobileNetV3-L and verify that it can benefit from TSM~\cite{lin2019tsm} by about 3\%. 


%As we increase the size of our models, we see that \ournet has the advantage of being more accurate at various efficiency thresholds.
There are more significant margins between larger \ournets (A3--A6) and their counterparts in the X3D family. 
It is not surprising because NAS should intuitively be more advantageous over the handcrafting method for X3D when the design space is large.  
\ournet-A5 and \ournet-A6 outperform several state-of-the-art video networks, including recent Transformer models like ViViT~\cite{arnab2021vivit} and TimeSformer~\cite{bertasius2021space} (see the last 6 rows of Table~\ref{table:k600-comparison}). 
\ournet-A6 with AutoAugment achieves 84.8\% accuracy (without pretraining) while still being substantially more efficient than comparable models (most often by an order of magnitude).
Even when compared to fully Transformer~\cite{vaswani2017attention} models like TimeSformer-HR~\cite{bertasius2021space}, \ournet-A6 outperforms it by 1\% accuracy and using 40\% of the FLOPs.

% We also compare with ResNet3D, (2+1)D ResNets implemented with feature gating \cite{he2016deep, tran2018closer, hara2018can, xie2017rethinking}, showing that our models provide an order of magnitude more efficiency.


\begin{table}[tbp]
    \begin{center}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}lrrrrrr@{}}
    % \begin{tabularx}{\columnwidth}{@{}Xrrrr@{}}
    \toprule
        \sc Model & \sc Top-1 & \sc Res & \sc Frames & \sc FPS & \sc gflops & \sc Mem (MB) \\
    \midrule
        MobileNetV3-L* \cite{howard2019searching} & \bf 68.1 & 224 & 1$\times$50 & 5 & 11.0 & \bf 23 \\
    \midrule
        \ournet-A0 & \bf 71.5 & 172 & 1$\times$50 & 5 & 2.71 & 173 \\
        \ournet-A0-Stream & 70.3 & 172 & 1$\times$50 & 5 & 2.73 & \bf 71 \\
    \midrule
        \ournet-A1 & \bf 76.0 & 172 & 1$\times$50 & 5 & 6.02 & 191 \\
        %\ournet-A1-Ens (x2) & 75.8 & 1$\times$25 & 2.5 & 125 & 98 \\
        \ournet-A1-Stream & 75.6 & 172 & 1$\times$50 & 5 & 6.06 & \bf 72 \\
        \ournet-A1-Stream-Ens (x2) & 75.9 & 172 & 1$\times$25 & 2.5 & 6.06 & \bf 72 \\
    \midrule
        \ournet-A2 & \bf 77.5 & 224 & 1$\times$50 & 5 & 10.3 & 470 \\
        \ournet-A2-Stream & 76.5 & 224 & 1$\times$50 & 5 & 10.4 & \bf 85 \\
        \ournet-A2-Stream-Ens (x2) & 77.0 & 224 & 1$\times$25 & 2.5 & 10.4 & \bf 85 \\
    \midrule
        \ournet-A3 & 80.8 & 256 & 1$\times$120 & 12 & 56.9 & 1310 \\
        %\ournet-A3-Ens (x2) & 80.7 & 224 & 1$\times$60 & 6 & 382 & 710 \\
        \ournet-A3-Stream & 79.6 & 256 & 1$\times$120 & 12 & 57.1 & \bf 82 \\
        \ournet-A3-Stream-Ens (x2) & \bf 80.4 & 256 & 1$\times$60 & 6 & 57.1 & \bf 82 \\
    \midrule
        \ournet-A4 & 81.2 & 290 & 1$\times$80 & 8 & 105 & 1390 \\
        \ournet-A4-Stream & 80.5 & 290 & 1$\times$80 & 8 & 106 & \bf 112 \\
        \ournet-A4-Stream-Ens (x2) & \bf 81.4 & 290 & 1$\times$40 & 4 & 106 & \bf 112 \\
    \midrule
        \ournet-A5 & 82.7 & 320 & 1$\times$120 & 12 & 281 & 2040 \\
        \ournet-A5-Stream & 82.0 & 320 & 1$\times$120 & 12 & 282 & \bf 171 \\
        \ournet-A5-Stream-Ens (x2) & \bf 82.9 & 320 & 1$\times$60 & 6 & 282 & \bf 171 \\
    \midrule
        ResNet3D-50 & \bf 78.7 & 224 & 1$\times$250 & 25 & 390 & 3040 \\
        ResNet3D-50-Stream & 76.9 & 224 & 1$\times$250 & 25 & 390 & \bf 2600 \\
        ResNet3D-50-Stream-Ens (x2) & 78.6 & 224 & 1$\times$125 & 12.5 & 390 & \bf 2600 \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \vspace{-2pt}
    \caption{
        {\bf Base vs. Streaming Architectures} on Kinetics 600.
        We and report the inference resolution (res), number of clips $\times$ frames per clip (frames), and frame rate (fps) for each video.
        We measure the total GFLOPs per video across all frames.
        % Frames indicates the number of frames embedded at a time.
        % MFLOPs measured in MFLOPs per frame.
        We denote ``Stream'' to be causal models using a stream buffer frame-by-frame, and ``Ens'' to be two ensembled models (with half the input frames so FLOPs are equivalent).
        Memory usage is measured in peak MB for a single video clip.
        * denotes our reproduced models.
        % \bg{Can we align the columns with those in Table~\ref{table:k600-comparison}? i.e., Top-1, GFLOPs (not MFLOPs), Res, Frames, FPS, Mem (MB). Also, bold the best number for each network in the Mem column.}
    }
    \label{table:balanced-vs-streaming}
    \vspace{-10pt}
\end{table}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/movinet_stream_memory_flops_joint_comparison_v2.pdf}
    \caption{
        {\bf Effect of Streaming \ournets on Memory} on Kinetics 600.
        Top left: comparison of accuracy vs. max memory usage on a V100 GPU on our models, progressively increasing in size.
        We evaluate two versions of \ournet: a base version without a stream buffer and a causal version with a stream buffer.
        Note that memory may be inflated due to padding and runtime overhead.
        Top right: comparison of max memory usage on a V100 GPU as a function of the number of input frames.
        Bottom: the classification accuracy.
        * denotes our reproduced models.
    }
    \label{fig:frame-stream}
    \vspace{-10pt}
\end{figure}



\vspace{-10pt}
\paragraph{\ournets with Stream Buffers.}
Our base \ournet architectures may consume lots of memory in the absence of modifications, especially as the model sizes and input frames grow.
Using the stream buffer with causal operations, we can have an order of magnitude peak memory reduction for large networks (\ournets A3-A6), as shown in the last column of Table~\ref{table:balanced-vs-streaming}.
% We see about a 1\% reduction in accuracy on Kinetics 600 across all models.
% However, memory consumption is significantly reduced when embedding all frames.
% E.g., \ournet-A1 must embed all 50 frames, while \ournet-A1-Stream uses smaller 1-frame window across those frames, resulting in a more than 50\% memory reduction.
% As models get larger, we see a much improved memory reduction in \ournet-A3 with nearly 6x less memory consumption as the base architecture.

Moreover, Figure~\ref{fig:frame-stream} visualizes the streaming architectures' effect on memory. 
From the left panel at the top, we see that our \ournets are more accurate and more memory-efficient across all model sizes compared to X3D, which employs multi-clip evaluation.  
We also demonstrate constant memory as we scale the total number of frames in the input receptive field at the top's right panel. 
The bottom panel indicates that the streaming \ournets remain efficient in terms of the GFLOPs per input video.

We also apply our stream buffer to ResNet3D-50 (see the last two rows in Table~\ref{table:balanced-vs-streaming}).
However, we do not see as much of a memory reduction, likely due to larger overhead when using full 3D convolution as opposed to the depthwise convolution in \ournets.

\vspace{-10pt}
\paragraph{\ournets with Stream Buffers and Ensembling.}
We see from Table~\ref{table:balanced-vs-streaming} only a small 1\% accuracy drop across all models after applying the stream buffer. 
We can restore the accuracy using the temporal ensembling without any additional inference cost.
Table~\ref{table:balanced-vs-streaming} reports the effect of ensembling two models trained at half the frame rate of the original model (so that GFLOPs remain the same). 
We can see the accuracy improvements in all streaming architectures, showing that ensembling can bridge the gap between streaming and non-streaming architectures, especially as model sizes grow.
It is worth noting that, unlike prior works, the ensembling balances accuracy and efficiency (GFLOPs) in the same spirit as~\cite{kondratyuk2020ensembling}, not just to boost the accuracy.
% \ournet-A3-Stream-Ens is comparable in accuracy to \ournet-A3, showing that ensembles can bridge the gap between streaming and non-streaming architectures, especially as model sizes grow.

\begin{figure*}[tbp]
    \begin{center}
    \includegraphics[width=1.0\linewidth]{images/movinet_all_joint_comparison_v3.pdf}
    \end{center}
    \vspace{-8pt}
    \caption{
        {\bf Accuracy vs. FLOPs Comparison} across 5 large-scale action recognition datasets.
        Each series represents a model family, with points representing individual models ordered by FLOPs.
        We report FLOPs per video using single-clip evaluation for all \ournets and compare with competitive multi-clip (and reproduced single-clip) models, using a log-scale on the x-axis.
        * denotes reproduced models.
        For Charades, we evaluate on MoViNet A1, A4, A5, and A6 only.
    }
    \label{fig:all-flops-comparison}
    \vspace{-10pt}
\end{figure*}

\subsection{Comparison Results on Other Datasets}

Figure~\ref{fig:all-flops-comparison} summarizes the main results of \ournets on all the five datasets along with state-of-the-art models that have results reported on the respective datasets. We compare \ournets with X3D~\cite{feichtenhofer2020x3d}, MSNet~\cite{kwon2020motionsqueeze}, TSM~\cite{lin2019tsm}, ResNet3D~\cite{he2016deep}, SlowFast~\cite{feichtenhofer2019slowfast}, EfficientNet-L2~\cite{xie2020self}, TVN~\cite{piergiovanni2020tiny}, SRTG~\cite{stergiou2020learn}, and AssembleNet~\cite{ryoo2019assemblenet, ryoo2020assemblenetpp}.
Appendix~\appendixmoreresults tabulates the results with more details.

Despite only searching for efficient architectures on Kinetics 600, NAS yields models that drastically improve over prior work on other datasets as well.
On Moments in Time, our models are 5-8\% more accurate than Tiny Video Networks (TVNs)~\cite{piergiovanni2020tiny} at low GFLOPs, and \ournet-A5 achieves 39.9\% accuracy, outperforming AssembleNet~\cite{ryoo2019assemblenet} (34.3\%) which uses optical flow as additional input (while our models do not).
On Charades, \ournet-A5 achieves the accuracy of 63.2\%, beating AssembleNet++~\cite{ryoo2020assemblenetpp} (59.8\%) which uses optical flow and object segmentation as additional inputs.
Results on Charades provide evidence that our models are also capable of sophisticated temporal understanding, as these videos can have longer duration clips than what is seen in Kinetics and Moments in Time.
% These results all point to unprecedented efficiency scaling, demonstrating the effectiveness and cross-dataset generalization of \ournets.


\subsection{Additional Analyses}

% \vspace{-5pt}
\paragraph{\ournet Operations.} We provide some ablation studies about
some critical \ournet operations in Table~\ref{table:stream-ablation}.
For the base network without the stream buffer, SE is vital for achieving high accuracy; \ournet-A1's accuracy drops by 2.9\% if we remove SE. 
We see a much larger accuracy drop when using CausalConv without SE than CausalConv with a global SE, which indicates that the global SE can take some of the role of standard Conv to extract information from future frames.
However, when we switch to a fully streaming architecture with CausalConv and CausalSE, this information from future frames is no longer available, and we see a large drop in accuracy, but still significantly improved from CausalConv without SE.
Using PosEnc, we can gain back some accuracy in the causal model.

\begin{table}[tbp]
    \centering
    \newcommand{\ck}{\checkmark}
    % \footnotesize
    \begin{center}
    \resizebox{0.9\columnwidth}{!}{%
    \begin{tabular}{@{}lcccccc@{}}
    % \begin{tabularx}{\columnwidth}{@{}Xrrrrrr@{}}
    \toprule
       \sc Model & \sc CausalConv & \sc SE & \sc CausalSE & \sc PosEnc & \sc Top-1 & \sc gflops \\
    \midrule
                   &     &     &     &     & 73.3 & \bf 6.04 \\
                   & \ck &     &     &     & 72.1 & \bf 6.04 \\
                   & \ck &     & \ck &     & 73.5 & 6.06 \\
        \ournet-A1 & \ck &     & \ck & \ck & 74.0 & 6.06 \\
                   & \ck & \ck &     &     & 74.9 & 6.06 \\
                   &     & \ck &     &     & \bf 75.2 & 6.06 \\
                %   &     &     & \ck & \ck & \bf 75.4 & 6.06 \\
    \midrule
                   &     &     &     &     & 77.7 & \bf 56.9 \\
        \ournet-A3 & \ck &     & \ck &     & 79.0 & 57.1 \\
                   & \ck &     & \ck & \ck & 79.6 & 57.1 \\
                   &     & \ck &     &     & \bf 80.3  & 57.1 \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \vspace{-2pt}
    \caption{
        {\bf \ournet Operations Ablation} on Kinetics 600.
        We compare different configurations on \ournet-A1, including Conv/CausalConv, SE/CausalSE/No SE, and PosEnc, and report accuracy and GFLOPs per video.
        % \zhl{Is the ablation conclusion the same for bigger models?}
    }
    \label{table:stream-ablation}
    \vspace{-10pt}
\end{table}

\begin{table}[t]
    % Architecture diagram commands
    \newcommand{\blocks}[3]{
        \multirow{3}{*}{
            \(\left[
            \begin{array}{c}
                \text{1$\times$1$^\text{2}$, #2}\\[-.1em] 
                \text{1$\times$3$^\text{2}$, #2}\\[-.1em] 
                \text{1$\times$1$^\text{2}$, #1}
            \end{array}
            \right]\)$\times$#3
        }
    }
    \newcommand{\blocket}[4]{\multirow{3}{*}{\(\left[\begin{array}{c}\text{1$\times$1$^\text{2}$, #1}\\[-.1em] \text{$3$$\times$3$^\text{2}$, #2}\\[-.1em] \text{1$\times$1$^\text{2}$, #3}\end{array}\right]\)$\times$#4}
    }
    \newcommand{\blockt}[3]{\multirow{3}{*}{\(\left[\begin{array}{c}\text{\underline{3$\times$1$^\text{2}$}, #2}\\[-.1em] \text{1$\times$3$^\text{2}$, #2}\\[-.1em] \text{1$\times$1$^\text{2}$, #1}\end{array}\right]\)$\times$#3}
    }
    % \newcommand{\blocke}[1]{}
    \newcommand{\blockseq}[3]{\text{#1$\times$#2$^\text{2}$, #3}\\[-.1em]}

    \begin{center}
    \resizebox{0.7\columnwidth}{!}{%
    % \begin{tabular}{@{}lcl@{}}
    % \small
    \begin{tabularx}{1.0 \columnwidth}{@{}Xcl@{}}
        \toprule
        \sc Stage & \sc Operation & \sc Output size \\
        \midrule
        data & stride 5, RGB & $50\times224^\text{2}$ \\
        conv$_1$ & \multicolumn{1}{c}{$1\times3^\text{2}$, {16}}
        & $50\times112^\text{2}$ \\
        \midrule
        % & \multirow{2}{*}{50\times112^\text{2}$}  \\
        % & stride \textbf{2}, 2$^\text{2}$ & \\
        block$_2$ & \multirow{3}{*}{
            \(\left[
            \begin{array}{c}
                \blockseq{{1}}{{5}}{{16, 40}}
                \blockseq{{3}}{{3}}{{16, 40}}
                \blockseq{{3}}{{3}}{{16, 64}}
            \end{array}
            \right]\)} & 
            \multirow{3}{*}{$50\times56^\text{2}$}  \\
        % \multirow{3}{*}{block$_1$} & \blocks{{16}}{{40}}{1} & \multirow{3}{*}{50\times56^\text{2}$}  \\
        &  & \\
        &  & \\
        block$_3$ & \multirow{5}{*}{
            \(\left[
            \begin{array}{c}
                \blockseq{{3}}{{3}}{{40, 96}}
                \blockseq{{3}}{{3}}{{40, 120}}
                \blockseq{{3}}{{3}}{{40, 96}}
                \blockseq{{3}}{{3}}{{40, 96}}
                \blockseq{{3}}{{3}}{{40, 120}}
            \end{array}
            \right]\)} & 
            \multirow{5}{*}{$50\times28^\text{2}$}  \\
        &  & \\
        &  & \\
        &  & \\
        &  & \\
        block$_4$ & \multirow{5}{*}{
            \(\left[
            \begin{array}{c}
                \blockseq{{5}}{{3}}{{72, 240}}
                \blockseq{{3}}{{3}}{{72, 155}}
                \blockseq{{3}}{{3}}{{72, 240}}
                \blockseq{{3}}{{3}}{{72, 192}}
                \blockseq{{3}}{{3}}{{72, 240}}
            \end{array}
            \right]\)} & 
            \multirow{5}{*}{$50\times14^\text{2}$}  \\
        &  & \\
        &  & \\
        &  & \\
        &  & \\
        block$_5$ & \multirow{6}{*}{
            \(\left[
            \begin{array}{c}
                \blockseq{{5}}{{3}}{{72, 240}}
                \blockseq{{3}}{{3}}{{72, 240}}
                \blockseq{{3}}{{3}}{{72, 240}}
                \blockseq{{3}}{{3}}{{72, 240}}
                \blockseq{{1}}{{5}}{{72, 144}}
                \blockseq{{3}}{{3}}{{72, 240}}
            \end{array}
            \right]\)} & 
            \multirow{6}{*}{$50\times14^\text{2}$}  \\
        &  & \\
        &  & \\
        &  & \\
        &  & \\
        &  & \\
        block$_6$ & \multirow{7}{*}{
            \(\left[
            \begin{array}{c}
                \blockseq{{5}}{{3}}{{144, 480}}
                \blockseq{{1}}{{5}}{{144, 384}}
                \blockseq{{1}}{{5}}{{144, 384}}
                \blockseq{{1}}{{5}}{{144, 480}}
                \blockseq{{1}}{{5}}{{144, 480}}
                \blockseq{{3}}{{3}}{{144, 480}}
                \blockseq{{1}}{{3}}{{144, 576}}
            \end{array}
            \right]\)} & 
            \multirow{7}{*}{$50\times7^\text{2}$}  \\
        &  & \\
        &  & \\
        &  & \\
        &  & \\
        &  & \\
        &  & \\
        % \midrule
        % \multirow{3}{*}{block$_3$} & \blockt{{1024}}{{256}}{5} & \multirow{3}{*}{$50\times14^\text{2}$} \\
        % &  & \\
        % &  & \\
        \midrule
        conv$_7$ & \multicolumn{1}{c}{$1\times1^\text{2}$, {640}}
        & $50\times7^\text{2}$ \\
        pool$_8$ & \multicolumn{1}{c}{$50\times7^\text{2}$}
        & $1\times1^\text{2}$ \\
        dense$_9$ & \multicolumn{1}{c}{$1\times1^\text{2}$, {2048}}
        & $1\times1^\text{2}$ \\
        dense$_{10}$ & \multicolumn{1}{c}{$1\times1^\text{2}$, {600}}
        & $1\times1^\text{2}$ \\
        \bottomrule
    \end{tabularx}
    % \end{tabular}
    }
    \end{center}
    \vspace{-5pt}
    \caption{
        {\bf \ournet-A2 Architecture} searched by TuNAS, running 50 frames on Kinetics 600.
        See Table~\ref{table:nas-ssd} for the search space definition detailing the meaning of each component.
    }
    \label{table:a2-architecture}
    \vspace{-10pt}
\end{table}


\vspace{-10pt}
\paragraph{\ournet Architectures.}
%Our NAS setup provides a strong method to produce highly efficient networks based on balancing spatiotemporal representations in each bottleneck block.
We provide the architecture description of \ournet-A2 in Table~\ref{table:a2-architecture} --- Appendix~\appendixarchitectures has the detailed architectures of other \ournets.
Most notably, the network prefers large bottleneck width multipliers in the range [2.5, 3.5], often expanding or shrinking them after each layer.
In contrast, X3D-M with similar compute requirements has a wider base feature width with a smaller constant bottleneck multiplier of 2.25.
The searched network prefers balanced 3x3x3 kernels, except at the first downsampling layers in the later blocks, which have 5x3x3 kernels.
The final stage almost exclusively uses spatial kernels of size 1x5x5, indicating that high-level features for classification benefit from mostly spatial features.
This comes at a contrast to S3D~\cite{xie2018rethinking}, which reports improved efficiency when using 2D convolutions at lower layers and 3D convolutions at higher layers.
% As a final outcome, the search produces an architecture that has 50\% of the FLOPs single-clip X3D-M, yet 0.6\% more accurate.

% \vspace{-10pt}
% \paragraph{\ournet Hardware Benchmarks.} For benchmarks running on real hardware, see Appendix~\appendixmoreresults.

%------------------------------------------------------------------------
\vspace{-10pt}
\subsubsection{Hardware Benchmark}

% \vspace{-10pt}
\ournets A0, A1, and A2 represent the fastest models that would most realistically be used on mobile devices.
% We compare them with MobileNetV3 in Figure~\ref{fig:mobile-comparison} with respect to both FLOPs and estimated latency on a Pixel 1 CPU.
We compare them with MobileNetV3 in Figure~\ref{fig:x86-comparison} with respect to both FLOPs and real-time latency on an x86 Intel Xeon W-2135 CPU at 3.70GHz.
These models are comparable in per-frame computation cost, as we evaluate on 50 frames for all models.
% From these results we can conclude that streaming \ournets can run faster on mobile phones while being more accurate at the same time, even with temporal modifications like TSM.
From these results we can conclude that streaming \ournets can run faster on CPU while being more accurate at the same time, even with temporal modifications like TSM.
While there is a discrepancy between FLOPs and latency, searching over a latency target explicitly in NAS can reduce this effect.
However, we still see that FLOPs is a reasonable proxy metric for CPU latency, which would translate well for mobile devices.
% However, we still see that FLOPs is a reasonable proxy metric for CPU latency on mobile devices.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/movinet_k600_x86_flops_latency_comparison_v2.pdf}
    \caption{
        {\bf CPU Latency Comparison} on Kinetics 600.
        We compare the efficiency of \ournets  (A0, A1, A2) vs. MobileNetV3~\cite{howard2019searching} using FLOPs and benchmarked latency on an x86 Xeon CPU at 3.70GHz.
    }
    \label{fig:x86-comparison}
\end{figure}

\begin{table}[t]
    \begin{center}
    \newcommand{\ck}{\checkmark}
    \newcommand{\xmark}{\ding{55}}
    % \footnotisize
    \resizebox{250pt}{!}{%
    \begin{tabular}{@{}lcrrr@{}}
    % \begin{tabular}{@{}ccccc@{}}
    \toprule
        \sc Model & \sc Streaming & \sc Video (ms) & \sc Frame (ms) & \sc Top-1 \\
    \midrule
        MoViNet-A0-Stream & \ck & 183 & 3.7 & 70.3 \\
        MoViNet-A1-Stream & \ck & 315 & 6.3 & 75.6 \\
        MoViNet-A2-Stream & \ck & 325 & 6.5 & 76.5 \\
        MoViNet-A3-Stream & \ck & 1110 & 9.2 & 79.6 \\
        MoViNet-A4-Stream & \ck & 1130 & 14.1 & 80.5 \\
        MoViNet-A5-Stream & \ck & 2310 & 19.2 & 82.0 \\
    \midrule
        MobileNetV3-S* & \ck & 68 & 1.4 & 61.3 \\
        MobileNetV3-L* & \ck & 81 & 1.6 & 68.1 \\
    \midrule
        X3D-M* (Single Clip) & \xmark  & 345 & 6.9 & 76.9 \\
        X3D-XL* (Single Clip) & \xmark & 943 & 18.9 & 80.3 \\
        % X3D-M* (Multi-Clip) & 6160 & 12.8 & 78.8 \\
        % X3D-XL* (Multi-Clip) & 15000 & 31.3 & 81.9 \\
    \bottomrule
    \end{tabular}
    }
    \end{center}
    \caption{
        {\bf Runtime on an Nvidia V100 GPU on Kinetics 600}. Latency is given for the entire video clip and per frame in ms. * denotes reproduced models.
    }
    \label{table:runtime-v100-comparison}
    \vspace{-10pt}
\end{table}

We also show benchmarks for \ournets running on an Nvidia V100 GPU in Table~\ref{table:runtime-v100-comparison}.
Similar to mobile CPU, our streaming model latency is comparable to single-clip X3D models.
However, we do note that MobileNetV3 can run faster than our networks on GPU, showing that the FLOPs metric for NAS has its limitations.
\ournets can be made more efficient by targeting real hardware instead of FLOPs, which we leave for future work.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=1.0\linewidth]{images/movinet_k600_mobile_flops_latency_comparison.pdf}
%     \caption{
%         {\bf Mobile Model Comparison} on Kinetics 600.
%         We compare the efficiency of \ournets vs. MobileNetV3~\cite{howard2019searching} using FLOPs and estimated latency on a Pixel 1 CPU.
%     }
%     \label{fig:mobile-comparison}
% \end{figure}

==> Mobile Video Networks Arxiv/sections/05_conclusion.tex <==
\ournets provide a highly efficient set of models that transfer well across different video recognition datasets.
Coupled with stream buffers, \ournets significantly reduce training and inference memory cost while also supporting online inference on streaming video.
We hope our approach to designing \ournets can provide improvements to future and existing models, reducing memory and computation costs in the process. 
% In future work, we will investigate the generalization abilities of \ournets to other video tasks like object detection and segmentation.
% We believe these approaches will produce significant efficiency gains for video models across a wide range of tasks.

